K-Means Clustering on Noisy Intermediate Scale Quantum Computers

Real-time clustering of big performance data generated by the telecommunication networks requires domain-specific high performance compute infrastructure to detect anomalies. In this paper, we evaluate noisy intermediate-scale quantum (NISQ) computers characterized by low decoherence times, for K-means clustering and propose three strategies to generate shorter-depth quantum circuits needed to overcome the limitation of NISQ computers. The strategies are based on exploiting; i) quantum interference, ii) negative rotations and iii) destructive interference. By comparing our implementations on IBMQX2 machine for representative data sets, we show that NISQ computers can solve the K-means clustering problem with the same level of accuracy as that of classical computers.

==> figures/qcircuit_2qubit_distance.tex <==
\begin{equation*}
    \Qcircuit @C=1.0em @R=2.0em {
    & & & & & \ustick{A} & & & & & & & & \ustick{B} \\
	 \lstick{\ket{q_1}: \ket{0} } & \gate{H} & \ctrl{1} & \qw  &  \ctrl{1} & \gate{X} & \qw & \ctrl{1} & \qw & \ctrl{1} & \qw  &  \qw &\gate{H} & \qw &\meter\\
	 \lstick{\ket{q_2}: \ket{0} } & \qw & \targ  & \gate{R_y(-\theta_t)} & \targ & \gate{R_y(\theta_t)} & \qw & \targ & \gate{R_y(-\theta_{c})} & \targ & \gate{R_y(\theta_{c})} & \qw & \qw  & \qw & \qw  \gategroup{2}{2}{3}{11}{1.0em}{--} \gategroup{2}{13}{3}{15}{1.0em}{^\}}
	 }
\end{equation*}

==> figures/qcircuit_2qubit_distance_optimized.tex <==
\begin{equation*}
    \Qcircuit @C=1.0em @R=2.0em {
     & & & \ustick{A} & & & & & \ustick{B} \\
	 \lstick{\ket{q_1}: \ket{0} } & \gate{H} & \ctrl{1} & \qw  &  \ctrl{1} & \qw & \qw  & \gate{H} & \qw &  \meter\\
	 \lstick{\ket{q_2}: \ket{0} } & \qw & \targ  & \gate{R_y(-|\theta_t - \theta_{c}|)} & \targ & \gate{R_y(|\theta_t - \theta_{c}|)} & \qw  & \qw & \qw & \qw \gategroup{2}{2}{3}{6}{1.0em}{--} \gategroup{2}{8}{3}{10}{1.0em}{^\}}
	 }
\end{equation*}

==> figures/qcircuit_basic_implementation_1.tex <==
\begin{equation*}
    \Qcircuit @C=1.0em @R=1.0em {
        & & & \ustick{B} & & & & & & & & &  \ustick{C}\\
	 	\lstick{\ket{a_0}: \ket{0} } & \gate{H} & \ctrl{2} & \qw  &  \ctrl{2} & \gate{X} & \qw & \ctrl{1} & \qw & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \qw & \rstick{\ket{a_1}} \qw\\
	 	\lstick{\ket{i_0}: \ket{0}} & \gate{H} & \qw & \qw & \qw & \qw & \qw  & \ctrl{1} & \ctrl{1} & \qw & \ctrl{1} & \qw & \ctrl{1} & \ctrl{1} & \qw & \ctrl{1} & \gate{X}  & \rstick{\ket{i_1}} \qw\\
	 	\lstick{\ket{d_0}: \ket{0}} & \qw & \targ  & \gate{R_y(-\theta_t)} & \targ & \gate{R_y(\theta_t)} & \qw & \targ & \targ & \gate{R_y(\frac{\theta_{c_1}}{2})} & \targ & \gate{R_y(\frac{-\theta_{c_1}}{2})} & \targ & \targ & \gate{R_y(\frac{-\theta_{c_1}}{2})} & \targ & \gate{R_y(\frac{\theta_{c_1}}{2})} & \rstick{\ket{d_1}} \qw\\
	 	\lstick{\ket{c_0}: \ket{0}} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \rstick{\ket{c_1}} \qw \gategroup{2}{3}{4}{6}{1.0em}{--} \gategroup{2}{8}{4}{17}{1.0em}{--}
	 }
\end{equation*}

==> figures/qcircuit_basic_implementation_2.tex <==
\begin{equation}
    \Qcircuit @C=1.0em @R=1.0em {
        & & & & & & \ustick{D} & & & & & & \ustick{E} & & \ustick{F} \\
	 	\lstick{\ket{a_1}} & \ctrl{1} & \qw & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \qw & \qw & \qw & \gate{H} & \meter\\
	 	\lstick{\ket{i_1}} & \ctrl{1} & \ctrl{1} & \qw & \ctrl{1} & \qw & \ctrl{1} & \ctrl{1} & \qw & \ctrl{1} & \qw & \qw & \ctrl{2} & \qw & \meter \\
	 	\lstick{\ket{d_1}}  & \targ & \targ & \gate{R_y(\frac{\theta_{c_2}}{2})} & \targ & \gate{R_y(\frac{-\theta_{c_2}}{2})} & \targ & \targ & \gate{R_y(\frac{-\theta_{c_2}}{2})} & \targ & \gate{R_y(\frac{\theta_{c_2}}{2})} &\qw & \qw & \qw &  \meter\\
	 	\lstick{\ket{c_1}}  & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw  & \qw & \targ & \qw & \meter \gategroup{2}{2}{4}{11}{1.0em}{--}
	 	\gategroup{3}{13}{5}{13}{1.0em}{--}
	 	\gategroup{2}{14}{2}{15}{1.0em}{^)}
	 }
\end{equation}

==> figures/qcircuit_negative_rotations_4.tex <==
\begin{equation*}
    \Qcircuit @C=1.0em @R=1.5em {
	 	\lstick{\ket{q_1}: \ket{0}} & \gate{R_y(\theta_t)} & \qw & \gate{R_y(-\theta_{c_1})} & \meter\\
	 	\lstick{\ket{q_2}: \ket{0}} & \gate{R_y(\theta_t)} & \qw & \gate{R_y(-\theta_{c_2})} & \meter\\
	 	\lstick{\ket{q_3}: \ket{0}} & \gate{R_y(\theta_t)} & \qw & \gate{R_y(-\theta_{c_3})} & \meter & \rstick{t_{cluster} = Index\left( max(P\ket{0}_{q_1}...P\ket{0}_{q_k}) \right)}\\
	 	\lstick{\ket{q_4}: \ket{0}} & \gate{R_y(\theta_t)} & \qw & \gate{R_y(-\theta_{c_4})} & \meter\\
	 	\cds{0}{\vdots} \\
	 	\lstick{\ket{q_k}: \ket{0}} & \gate{R_y(\theta_t)} & \qw & \gate{R_y(-\theta_{c_k})} & \meter \gategroup{1}{1}{6}{5}{1.0em}{\}}\\
	 }
\end{equation*}

==> figures/qcircuit_negative_rotations_nk.tex <==
\begin{equation*}
    \Qcircuit @C=1.0em @R=1.5em {
	 	\lstick{\ket{q_1}: \ket{0}} & \gate{R_y(\theta_{t_1})} & \qw & \gate{R_y(-\theta_{c_1})} & \meter\\
	 	\lstick{\ket{q_2}: \ket{0}} & \gate{R_y(\theta_{t_1})} & \qw & \gate{R_y(-\theta_{c_2})} & \meter & \rstick{t_{1_{cluster}} = Index\left( max(P\ket{0}_{q_1}...P\ket{0}_{q_k}) \right)}\\
	 	\cds{0}{\vdots}  \\
	 	\lstick{\ket{q_k}: \ket{0}} & \gate{R_y(\theta_{t_1})} & \qw & \gate{R_y(-\theta_{c_k})} & \meter\\
	 	\cds{0}{\vdots} \\
	 	\cds{0}{\vdots} \\
	 	\lstick{\ket{q_{k(n-1)}}: \ket{0}} & \gate{R_y(\theta_{t_n})} & \qw & \gate{R_y(-\theta_{c_1})} & \meter\\
	 	\lstick{\ket{q_{k(n-1)+1}}: \ket{0}} & \gate{R_y(\theta_{t_n})} & \qw & \gate{R_y(-\theta_{c_2})} & \meter & \rstick{t_{n_{cluster}} = Index\left( max(P\ket{0}_{q_{k(n-1)}}...P\ket{0}_{q_{nk}}) \right)} \\
	 	\cds{0}{\vdots} \\
	 	\lstick{\ket{q_{nk}}: \ket{0}} & \gate{R_y(\theta_{t_n})} & \qw & \gate{R_y(-\theta_{c_k})} & \meter \gategroup{1}{1}{4}{5}{1.0em}{\}} \gategroup{7}{1}{10}{5}{1.0em}{\}}
	 }
\end{equation*}

==> figures/qcircuit_optimized_4.tex <==
\begin{equation*}
    \Qcircuit @C=0.8em @R=1.0em {
	 	\lstick{\ket{a_0}: \ket{0} } & \gate{H} & \ctrl{2} & \qw  &  \ctrl{2} & \gate{X} & \qw & \ctrl{1} & \qw & \qw & \ctrl{1} & \qw & \ctrl{1} & \qw & \qw & \ctrl{1} & \qw & \gate{H} & \meter\\
	 	\lstick{\ket{i_0}: \ket{0}} & \gate{H} & \qw & \qw & \qw & \qw & \qw  & \ctrl{1} & \ctrl{1} & \qw & \ctrl{1} & \gate{X} & \ctrl{1} & \ctrl{1} & \qw & \ctrl{1} & \ctrl{2} & \qw  & \meter \\
	 	\lstick{\ket{d_0}: \ket{0}} & \qw & \targ  & \gate{R_y(-\theta_t)} & \targ & \gate{R_y(\theta_t)} & \qw & \targ & \targ & \gate{R_y(\theta_{c_1})} & \targ & \qw & \targ & \targ & \gate{R_y(\theta_{c_2})} & \targ & \qw & \qw & \meter \\
	 	\lstick{\ket{c_0}: \ket{0}} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw &  \meter
	 }
\end{equation*}

==> figures/qcircuit_swap.tex <==
\begin{equation*}
    \Qcircuit @C=1.0em @R=1.0em @!R @!C {
	 	\lstick{\ket{0}} & \gate{H} & \ctrl{1} & \gate{H} &  \meter & \cw \\
	 	\lstick{\ket{a}} & \qw &  \qswap & \qw & \qw & \qw\\
	 	\lstick{\ket{b}} & \qw &  \qswap \qwx & \qw & \qw & \qw\\
	 }
\end{equation*}

==> figures/qcircuit_swap_gate_.breakdown.tex <==
\begin{equation*}
    \Qcircuit @C=1.0em @R=0.9cm {
	 	  &  \qswap & \qw  \\
	 	  &  \qswap \qwx & \qw  \\
    }
    \ \ \ \ \ \ \ \ 
    \Qcircuit @C=1.0em @R=0.5cm {
	 	  &  \ctrl{1} & \gate{H} & \ctrl{1} & \gate{H} & \ctrl{1} & \qw  \\
	 	  &  \targ & \gate{H} & \targ & \gate{H} & \targ & \qw \\
    }
\end{equation*}

==> figures/state_transition_flowchar_c2.tex <==
% Define block styles
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{decision} = [diamond, minimum width=2cm, minimum height=0.5cm, text centered, draw=black,]
\tikzstyle{arrow} = [thick,->,>=stealth]
    
\begin{tikzpicture}[node distance=2cm]
%nodes
\node (init) [startstop] {Input vector: $c_2$};
\node (start) [startstop, below of=init] {Rotate: $\left( \frac{\theta_{c_1}}{2}\right)$};
\node (input) [startstop, below of=start] {X: NOT};
\node (state_preparation) [startstop, below of=input] {Rotate: $\left( -\frac{\theta_{c_2}}{2}\right)$};


%arrows
\draw [arrow] (init) -- (start);
\draw [arrow] (start) -- (input);
\draw [arrow] (input) -- (state_preparation);





%\draw [arrow] (dec1) -- node[right] {yes} (pro2a);
%\draw [arrow] (dec1) -- node[above] {no} (pro2b);

%\draw[arrow] (pro2a) -- (out1);
%\draw[arrow] (out1) -- (stop);



\end{tikzpicture}

==> figures/state_transition_flowchar_t1.tex <==
% Define block styles
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{decision} = [diamond, minimum width=2cm, minimum height=0.5cm, text centered, draw=black,]
\tikzstyle{arrow} = [thick,->,>=stealth]
    
\begin{tikzpicture}[node distance=2cm]
%nodes
\node (init) [startstop] {Input vector: $t'$};
\node (start) [startstop, below of=init] {Rotate: $\theta_t$};
\node (input) [startstop, below of=start] {Rotate: $\left( \frac{\theta_{c_1}}{2}\right)$};
\node (state_preparation) [startstop, below of=input] {X: NOT};
\node (last) [startstop, below of=state_preparation] {Rotate: $\left( \frac{\theta_{c_2}}{2}\right)$};


%arrows
\draw [arrow] (init) -- (start);
\draw [arrow] (start) -- (input);
\draw [arrow] (input) -- (state_preparation);
\draw [arrow] (state_preparation) -- (last);

\end{tikzpicture}

==> figures/state_transition_flowchart_c1.tex <==
% Define block styles
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{decision} = [diamond, minimum width=2cm, minimum height=0.5cm, text centered, draw=black,]
\tikzstyle{arrow} = [thick,->,>=stealth]
    
\begin{tikzpicture}[node distance=2cm]
%nodes
\node (init) [startstop] {Input vector: $c_1$};
\node (start) [startstop, below of=init] {X: NOT};
\node (input) [startstop, below of=start] {Rotate: $\left(- \frac{\theta_{c_1}}{2}\right)$};
\node (state_preparation) [startstop, below of=input] {Rotate: $\left( \frac{\theta_{c_2}}{2}\right)$};


%arrows
\draw [arrow] (init) -- (start);
\draw [arrow] (start) -- (input);
\draw [arrow] (input) -- (state_preparation);





%\draw [arrow] (dec1) -- node[right] {yes} (pro2a);
%\draw [arrow] (dec1) -- node[above] {no} (pro2b);

%\draw[arrow] (pro2a) -- (out1);
%\draw[arrow] (out1) -- (stop);



\end{tikzpicture}

==> figures/state_transition_flowchart_t.tex <==



% Define block styles
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{decision} = [diamond, minimum width=2cm, minimum height=0.5cm, text centered, draw=black,]
\tikzstyle{arrow} = [thick,->,>=stealth]
    
\begin{tikzpicture}[node distance=2cm]
%nodes
\node (init) [startstop] {Input vector: $t$};
\node (start) [startstop, below of=init] {Rotate: $\theta_t$};
\node (input) [startstop, below of=start] {X: NOT};
\node (state_preparation) [startstop, below of=input] {Rotate: $\left( \frac{\theta_{c_1}}{2}\right)$};
\node (last) [startstop, below of=state_preparation] {Rotate: $\left( \frac{\theta_{c_2}}{2}\right)$};


%arrows
\draw [arrow] (init) -- (start);
\draw [arrow] (start) -- (input);
\draw [arrow] (input) -- (state_preparation);
\draw [arrow] (state_preparation) -- (last);





%\draw [arrow] (dec1) -- node[right] {yes} (pro2a);
%\draw [arrow] (dec1) -- node[above] {no} (pro2b);

%\draw[arrow] (pro2a) -- (out1);
%\draw[arrow] (out1) -- (stop);



\end{tikzpicture}



